From Two-Way to One-Way Finite State Transducers

Any two-way finite state automaton is equivalent to some one-way finite state automaton. This well-known result, shown by Rabin and Scott and independently by Shepherdson, states that two-way finite state automata (even non-deterministic) characterize the class of regular languages. It is also known that this result does not extend to finite string transductions: (deterministic) two-way finite state transducers strictly extend the expressive power of (functional) one-way transducers. In particular deterministic two-way transducers capture exactly the class of MSO-transductions of finite strings. In this paper, we address the following definability problem: given a function defined by a two-way finite state transducer, is it definable by a one-way finite state transducer? By extending Rabin and Scott's proof to transductions, we show that this problem is decidable. Our procedure builds a one-way transducer, which is equivalent to the two-way transducer, whenever one exists.

==> new.tex <==
\subsection{From \ZNFT to \NFT}


\begin{definition}[$\pptthree$-property]
  Let $T' \in \ZNFT$ with $m$ states, and let $(u,v)\in R(T')$ where
  $u$ has length $n$. Let $K = 2.o.m^3.|\Sigma|$ where $o = max\{|v|\
  |\ (p,a,v,q,m)\in \Delta\}$.  The pair $(u,v)$ satisfies the
  property $\pptthree$, denoted by $(u,v)\models \pptthree$, if for all
  accepting runs $\rho$ on $u$,
% such that $\out(\rho) = v$, 
    there exist two positions $1\leq \ell_1 \leq
  \ell_2 \leq n$ and $w,w',t_1,t_2,t_3\in \Sigma^*$ such that:
$$
\begin{array}{ll}
\out_1[1,\ell_1]   = w                            &  |t_i|\leq 3.K,\  \forall i\in \{1,2,3\}\\
\out_3[\ell_2,n+1] = w'                           &  |\out_1[\ell_2,n]| \leq 3.K \\
|\out_2[1,\ell_1]| \leq 3.K                       &  |\out_2[\ell_2,n]| \leq 3.K \\
\out_1[\ell_1,n]\out_2[1,n]\out_3[1,\ell_2] \in t_1t_2^*t_3   &  |\out_3[1,\ell_1]| \leq 3.K
\end{array}
$$
This decomposition is depicted in Fig.~\fbox{TODO}.
  $T'$ satisfies property $\pptthree$, denoted $T\models \pptthree$, if
  all $(u,v)\in R(T')$ satisfy it. 
\end{definition}


\begin{proposition}\label{prop:pptimpliesppttwo}
  Let $T'\in\ZNFT$. If $T'\models\ppt$, then $T'\models\pptthree$.
\end{proposition}

\begin{proof}
  We let $(i_1,i_2)$ be the leftmost loop such that
  $\out_2[i_1,i_2]\neq \varepsilon$ or
  $\out_3[i_1,i_2]\neq\varepsilon$. In particular, this implies that
  $|\out_2[1,i_1]|\leq K$ and $|\out_3[1,i_1]|\leq K$.  If such a loop
  does not exist, this implies that $|\out_2[1,n]|\leq K$ and
  $|\out_3[1,n+1]|\leq K$. This case is handled separately. We now
  assume the existence of this loop.

  Then, we let $(k_1,k_2)$ be the rightmost loop, verifying $k_1\geq
  i_2$, and such that $\out_1[k_1,k_2]\neq \varepsilon$ or
  $\out_2[k_1,k_2]\neq\varepsilon$. In particular, this implies that
  $|\out_1[k_2,n]|\leq K$ and $|\out_2[k_2,n]|\leq K$.  If such a loop
  does not exist, this implies that $|\out_1[i_2,n]|\leq K$ and
  $|\out_2[i_2,n]|\leq K$. This case is handled separately. We now
  assume the existence of this loop.

  





\end{proof}


\input{figures/singlecase}
